$(2+\epsilon)$-ANN for time series under the Fr\'echet distance

We study approximate-near-neighbor data structures for time series under the continuous Fr\'echet distance. For an attainable approximation factor $c>1$ and a query radius $r$, an approximate-near-neighbor data structure can be used to preprocess $n$ curves in $\mathbb{R}$ (aka time series), each of complexity $m$, to answer queries with a curve of complexity $k$ by either returning a curve that lies within Fr\'echet distance $cr$, or answering that there exists no curve in the input within distance $r$. In both cases, the answer is correct. Our first data structure achieves a $(5+\epsilon)$ approximation factor, uses space in $n\cdot \mathcal{O}\left({\epsilon^{-1}}\right)^{k} + \mathcal{O}(nm)$ and has query time in $\mathcal{O}\left(k\right)$. Our second data structure achieves a $(2+\epsilon)$ approximation factor, uses space in $n\cdot \mathcal{O}\left(\frac{m}{k\epsilon}\right)^{k} + \mathcal{O}(nm)$ and has query time in $\mathcal{O}\left(k\cdot 2^k\right)$. Our third positive result is a probabilistic data structure based on locality-sensitive hashing, which achieves space in $\mathcal{O}(n\log n+nm)$ and query time in $\mathcal{O}(k\log n)$, and which answers queries with an approximation factor in $\mathcal{O}(k)$. All of our data structures make use of the concept of signatures, which were originally introduced for the problem of clustering time series under the Fr\'echet distance. In addition, we show lower bounds for this problem. Consider any data structure which achieves an approximation factor less than $2$ and which supports curves of arclength up to $L$ and answers the query using only a constant number of probes. We show that under reasonable assumptions on the word size any such data structure needs space in $L^{\Omega(k)}$.

==> matching.tex <==

\begin{figure}
    %\centering
    \centering
\begin{tikzpicture}
    \draw[step=0.5, help lines, color=gray!30, dashed] (0,0) grid (5,5);
    \draw[->,ultra thick] (0,0)--(5,0) node[right]{$t$};
    \draw[->,ultra thick] (0,0)--(0,5) node[above]{$f(t)$};
    \draw[->,blue] (1,1.5) node[below]{$v_1$}--(3.2,3) node[below]{$v_2$};
    \draw[->,blue] (3.2,3)--(4,2.5) node[below]{$v_3$};
    \draw[->,red] (1,2) node[above]{$u_1$} --(3,3.5) node[above]{$u_2$};
     \draw[->,blue] (4,2.5)--(4.5,3) node[above]{$v_4$};
    \draw[->,red] (3,3.5)--(4.5,2.5) node[below]{$u_3$};
    \draw [decorate,decoration={brace,amplitude=4},xshift=0,yshift=0] (0.95,1.5) -- (0.95,2) node [black,midway,xshift=-0.5cm] { $1$};
   
    
    \end{tikzpicture}
    \hspace{2cm}
    \raisebox{1cm}{\includegraphics[page=3, width=0.25\textwidth]{freespace.pdf}}
    \caption{Left: An example of two signature curves and the matching constructed in the proof of Lemma~\ref{lemma:signtocurve}. The edge $\overline{v_1v_2}$ is matched with $\overline{u_1u_2}$, then $\overline{v_2v_3}$ is matched with $\overline{u_2u_3}$ and finally $\overline{v_3v_4}$ is matched with $u_3$; Right: The corresponding path in the free-space diagram of the two curves on the left. This is a \hl{tight matching} with the additional property that the horizontal and vertical segments of the path are restricted to cell boundaries.}
    \label{fig:matching}
\end{figure}

\begin{figure}
    \centering
    \includegraphics{2dtightmatching.pdf}
    \caption{Example of a  matching constructed in the proof of Lemma~\ref{lemma:signtocurve}. The left figure shows the two curves together with their signatures in bold lines. The right shows the free-space diagram with the  matching. The sections of the path in the $0$-free space are the diagonal edges: $\overline{(t_1,0),(t_2,p_1)}$, $\overline{(t_2,p_2)(t_3,p_3)}$, $\overline{(t_3,p_4)(t_4,p_5)}$, and a short diagonal edge that is not explicitly marked. The remainder of the path is uniquely defined by specifying these diagonal edges.}
    \label{fig:my_label}
\end{figure}
